Gaussian Processes Retrieval of LAI from Sentinel-2 Top-of-Atmosphere Radiance Data

Retrieval of vegetation properties from satellite and airborne optical data usually takes place after atmospheric correction, yet it is also possible to develop retrieval algorithms directly from top-of-atmosphere (TOA) radiance data. One of the key vegetation variables that can be retrieved from at-sensor TOA radiance data is the leaf area index (LAI) if algorithms account for variability in the atmosphere. We demonstrate the feasibility of LAI retrieval from Sentinel-2 (S2) TOA radiance data (L1C product) in a hybrid machine learning framework. To achieve this, the coupled leaf-canopy-atmosphere radiative transfer models PROSAIL-6S were used to simulate a look-up table (LUT) of TOA radiance data and associated input variables. This LUT was then used to train the Bayesian machine learning algorithms Gaussian processes regression (GPR) and variational heteroscedastic GPR (VHGPR). PROSAIL simulations were also used to train GPR and VHGPR models for LAI retrieval from S2 images at bottom-of-atmosphere (BOA) level (L2A product) for comparison purposes. The VHGPR models led to consistent LAI maps at BOA and TOA scale. We demonstrated that hybrid LAI retrieval algorithms can be developed from TOA radiance data given a cloud-free sky, thus without the need for atmospheric correction.

==> sentinel2.tex <==

Sentinel-2 (S2) is a satellite mission part of the European Commission's {\it Copernicus} programme, with the goal of monitoring of vegetation, soil and inland and coastal water areas for supporting agro-ecosystems applications \cite{Drusch2012}. Developed by the European Space Agency (ESA), S2 mission consists of a constellation of two satellites (S2A and S2B) that enables a global revisit time below 5 days.
S2's optical instrument -- the MultiSpectral Instrument (MSI) -- covers a wide swath (290 km) with high spatial resolution (10-60 m) in 13 spectral bands from the visible and NIR (VNIR) to SWIR spectral range. Further mission technical characteristics are summarized in Tab. \ref{tab:sensorchar} and Fig. \ref{fig:S2isrf} for band configuration.

\begin{table}[h]
\small
\centering
\caption{MSI/Sentinel-2 sensor characteristics as per \cite{s2techguide}.}
%\resizebox{0.90\linewidth}{!}{
\begin{tabular}{l l}
\hline
\textbf{Technical characteristics} 	& \textbf{Value} 		       \\ \hline
\textbf{Imaging principle}		    & Pushbroom-grating     	\\ 
\textbf{Spectral range [nm]}    	& 400--2200	nm      		\\ 
\textbf{Geolocation accuracy}   	& $<$12.5 m	        	 	\\ 
\textbf{SNR @L$_{ref}$}		    	& 50--175    	        	\\ 
\textbf{Radiometric accuracy}   	& 3\% abs, 1\% rel 	        \\ 
\textbf{A/D conversion}   	        & 12 bits        	        \\ 
\textbf{Coverage}			    	& Land and coastal areas 	\\ 
\hline
\end{tabular}
%}
\label{tab:sensorchar}
\end{table}

\begin{figure}[!ht]
	\centering
	\resizebox{0.8\textwidth}{!}{ 
	\IG[width=\linewidth]{figures/S2isrf.eps}
	\caption{MSI-S2A spectral response function for the 13 spectral bands used by the Ground Segment as from 15 January 2018~\cite{s2isrf}.}
	\label{fig:S2isrf}}
\end{figure}

The S2 MSI data is freely available from Copernicus Open Access Hub. From mid 2018 onwards, two reflectance products are provided: L1C and L2A. The L1C product refers TOA reflectances (i.e., TOA radiance normalized by incident solar irradiance). The L2A product refers to bottom-of-atmosphere (BOA) reflectance, which is achieved by means of the Sen2Cor atmospheric correction scheme (version 2.4.1)~\cite{MainKnorn2017}. 
Sen2Cor processing scheme is based on state-of-the-art algorithms that include cirrus cloud correction and scene classification~\cite{sen2corCirrus,sen2corCloud}. Sen2Cor relies on the Dark Dense Vegetation algorithm for the retrieval of aerosol type (rural/continental by default) and optical thickness \red{value at 550 nm (AOT$_{550}$)}~\cite{sen2corDDV}. The Atmospheric Pre-corrected Differential Absorption (APDA) algorithm is implemented for the retrieval of columnar water vapor (CWV)~\cite{SCHLAPFER1998353}.
Derivation of surface reflectance is achieved from the atmospheric inversion of a set of look-up tables generated with the libRadtran atmospheric RTM~\cite{emde2015}. 
Sen2Cor achieves uncertainties around 0.03 for the \red{AOT$_{550}$} and 0.3 g$\cdot$cm$^{-2}$ for the CWV, which are propagated to absolute errors of $<$0.05 in surface reflectance~\cite{Louis2016,rs9040322,Li20181997}. \red{These errors, nevertheless, should not hamper the retrieval of biophysical variables from L2A reflectance data, e.g. as successfully demonstrated by \cite{Vuolo2016,Djamai2019}.}




